Central Bank Digital Currency, Flight-to-Quality, and Bank-Runs in an Agent-Based Model

We analyse financial stability and welfare impacts associated with the introduction of a Central Bank Digital Currency (CBDC) in a macroeconomic agent-based model. The model considers firms, banks, and households interacting on labour, goods, credit, and interbank markets. Households move their liquidity from deposits to CBDC based on the perceived riskiness of their banks. We find that the introduction of CBDC exacerbates bank-runs and may lead to financial instability phenomena. The effect can be changed by introducing a limit on CBDC holdings. The adoption of CBDC has little effect on macroeconomic variables but the interest rate on loans to firms goes up and credit goes down in a limited way. CBDC leads to a redistribution of wealth from firms and banks to households with a higher bank default rate. CBDC may have negative welfare effects, but a bound on holding enables a welfare improvement.

==> tables/fb_bb_ntw_table.tex <==
\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{lccccc}
\toprule
  & mean & std & median & min & max \\
\midrule
banks links to firms & 0.0522 & 0.0569 & 0.0360 & 0.0000 & 0.7140 \\
banks links to banks (outdegree) & 0.0457 & 0.2089 & 0.0000 & 0.0000 & 1.0000 \\
banks links to banks (indegree) & 0.0771 & 0.2667 & 0.0000 & 0.0000 & 1.0000 \\
\bottomrule
\end{tabular}
\end{table}
